Bullseye: Structured Passage Retrieval and Document Highlighting for Scholarly Search

We present the Bullseye system for scholarly search. Given a collection of research papers, Bullseye: 1) identifies relevant passages using any on-the-shelf algorithm; 2) automatically detects document structure and restricts retrieved passages to user-specifed sections; and 3) highlights those passages for each PDF document retrieved. We evaluate Bullseye with regard to three aspects: system effectiveness, user effectiveness, and user effort. In a system-blind evaluation, users were asked to compare passage retrieval using Bullseye vs. a baseline which ignores document structure, in regard to four types of graded assessments. Results show modest improvement in system effectiveness while both user effectiveness and user effort show substantial improvement. Users also report very strong demand for passage highlighting in scholarly search across both systems considered.

==> RelatedWorks.tex <==
%FROM:Hildreth, C. R. (2001) Accounting for users? inflated assessments of on-line catalogue search performance and usefulness: an experimental study. Information Research.
%Hildreth et al.~\cite{hildreth2001accounting} argued that evaluation studies that relied on measures such as user perception of ease of use and subjective satisfaction with the search results did not provide a clear and consistent answer as to how user satisfaction may predict their actual search effectiveness. He found that user perception of ease of use had an effect, possibly greater than the results themselves, on user satisfaction.
Kamps et al.~\cite{kamps2003xml} listed two ways of Information Retrieval, which are {\em Full Document Retrieval } 
and {\em Element Retrieval }
%can be performed for text : 
%\begin{itemize}
%\item {\em Full Document Retrieval System } A baseline is formed by using a standard document index in which only whole documents are considered as a retrievable unit.
%\item {\em Element Retrieval System } The documents are indexed into retrieval units. Elements rather than documents then become the returned results of the user query. 
%\end{itemize}
In this paper, we concentrate on passage-level retrieval and highlight. In the measurement, we not only cover user perception of ease of use and satisfaction with the search results,
but also cover more objective metrics (e.g., exhaustivity and specificity as covered in Section~\ref{sec:evaluationSettings}).
%not very clear of how the works above are related to ours
%With our research we wish to establish that combination of document-level and passage-level improves user satisfaction.~\cite{model} ~\cite{kamps2003xml} 

Lalmas et al.~\cite{lalmas2007evaluating} mentioned two types of topics being identified by INEX,
where are {\em Content-only (CO) } and  {\em Content-and-structure (CAS)}.
%\begin{itemize}
%\item {\em Content-only (CO) } topics are requests that do not include reference to the document structure. They are traditional topics used in information retrieval test collections. However, the results to such topics are elements of various complexity, e.g. at different levels of the XML documents structure.
%\item {\em Content-and-structure (CAS)} topics are requests that contain conditions referring both to content and structure of a document. These conditions may refer to the content of specific elements, or may specify the type of the requested answer elements (e.g. sections should be retrieved).
%\end{itemize}
The baseline algorithm is closely related to answering queries in INEX Content-only(CO) topics where the user requests do not include reference to the document structure. The Bullseye algorithm is closely related to answering queries in INEX Content-and-structure topics where the user requests do contain conditions 
referring both to content and structure of document.

Cui et al.~\cite{cui2003hierarchical} proposed a new hierarchical index propagation and pruning mechanism for structured documents and realized a flexible element retrieval system based on this index structure. 
Their work was carried on XML documents, whereas our research focuses on PDF documents. 

Denny et al.~\cite{denny2009evaluation} designed a SecTag algorithm to identify both labeled and un-labeled (implied) note section headers in ``history and physical examination'' documents.
Their work calculated Bayesian probability for all of a document's section header candidates while our work is much more straightforward as each section header in a research paper is labeled. 
Our work of automatically identifying section headers is largely built upon the SecTag's method.
